Apiary: A DBMS-Integrated Transactional Function-as-a-Service Framework

Developers increasingly use function-as-a-service (FaaS) platforms for data-centric applications that perform low-latency and transactional operations on data, such as for microservices or web serving. Unfortunately, existing FaaS platforms support these applications poorly because they physically and logically separate application logic, executed in cloud functions, from data management, done in interactive transactions accessing remote storage. Physical separation harms performance while logical separation complicates efficiently providing transactional guarantees and fault tolerance. This paper introduces Apiary, a novel DBMS-integrated FaaS platform for deploying and composing fault-tolerant transactional functions. Apiary physically co-locates and logically integrates function execution and data management by wrapping a distributed DBMS engine and using it as a unified runtime for function execution, data management, and operational logging, thus providing similar or stronger transactional guarantees as comparable systems while greatly improving performance and observability. To allow developers to write complex stateful programs, we leverage this integration to enable efficient and fault-tolerant function composition, building a frontend for orchestrating workflows of functions with the guarantees that each workflow runs to completion and each function in a workflow executes exactly once. We evaluate Apiary against research and production FaaS platforms and show it outperforms them by 2--68x on microservice workloads by reducing communication overhead.

==> future_work.tex <==
\section{Discussion}
\label{sec:future_work}

We now describe potential future directions that further explore tight integration with the DBMS
to solve problems that are difficult in existing systems,
then discuss how future DBMSs could better support FaaS programming models.

\subsection{Possible Extensions}

\noindent\textbf{Privacy.}
Laws such as GDPR mandate that personally identifiable information (PII) can only be used for certain
purposes and must be deleted upon request~\cite{politou2018forgetting}.
There has already been much work on using DBMSs for privacy~\cite{gdprbench,istvan2021software},
and we believe the tight integration of data management with function execution in \sn can simplify the development of end-to-end privacy-preserving features.
For example, using DBMS access control, a function could be associated with specific purposes
and its access to application tables restricted based on those purposes.
Moreover, using \sn observability capabilities (Section~\ref{sec:provenance}), 
organizations could audit and monitor applications for privacy violations.

\noindent\textbf{Self-Adaptivity.}
There has been much recent research on applying machine learning (ML) to systems problems,
including scheduling~\cite{hongzi2019mlscheduling}, database index construction~\cite{10.1145/3183713.3196909,10.1145/3401071.3401659},
and DBMS configuration and tuning~\cite{10.1145/3035918.3064029,10.1145/3299869.3300085}.
A common challenge in these systems is collecting the data (e.g., system traces) needed for ML models and inference.
By leveraging tight integration of function execution and data management, we can extend \sn to capture more detailed information on both system and application behavior.


\subsection{DBMS Support for FaaS}

\noindent\textbf{Multi-Tenant Databases.}
Currently, \sn isolates applications by running each application in its own backend.
However, we may potentially increase resource utilization 
by running different applications in a multi-tenant database.
This requires solving two challenges.
First, performance isolation: leveraging prior work on fair scheduling in multi-tenant systems~\cite{pisces,das2013CPU} and real-time databases~\cite{abbott1992scheduling,haritsa1991earliest}
to ensure all FaaS applications receive only their fair share of cluster resources.
Second, security isolation: leveraging sandboxing research~\cite{shredder,firecracker,nacl} to isolate stored procedures containing arbitrary user code from one another and from the database.

\noindent\textbf{Cross-Datastore Transactions.}
\sn provides good performance and strong guarantees for applications accessing a single data store,
but some applications access multiple data stores, for example a relational database like Postgres
plus a text search system like Elasticsearch~\cite{laigner2021data}. In principle, \sn could be extended
to support multi-datastore backends, where some functions access one data store and other functions access another.
However, this requires cross-database transactions so that functions accessing different data stores could 
be grouped into a single transaction.  There has been much work on cross-database transactions, but much of it
either requires data stores to implement restrictive interfaces such as XA or is limited to specific APIs like key-value stores~\cite{cherrygarcia}.
We would benefit from a more general solution.
